ToMoBrush: Exploring Dental Health Sensing using a Sonic Toothbrush

Early detection of dental disease is crucial to prevent adverse outcomes. Today, dental X-rays are currently the most accurate gold standard for dental disease detection. Unfortunately, regular X-ray exam is still a privilege for billions of people around the world. In this paper, we ask: "Can we develop a low-cost sensing system that enables dental self-examination in the comfort of one's home?" This paper presents ToMoBrush, a dental health sensing system that explores using off-the-shelf sonic toothbrushes for dental condition detection. Our solution leverages the fact that a sonic toothbrush produces rich acoustic signals when in contact with teeth, which contain important information about each tooth's status. ToMoBrush extracts tooth resonance signatures from the acoustic signals to characterize varied dental health conditions of the teeth. We evaluate ToMoBrush on 19 participants and dental-standard models for detecting common dental problems including caries, calculus, and food impaction, achieving a detection ROC-AUC of 0.90, 0.83, and 0.88 respectively. Interviews with dental experts validate ToMoBrush's potential in enhancing at-home dental healthcare.

==> Evaluation.tex <==
\section{Results}\label{sec:results}


We present three categories of results: (1) \textbf{Health Detection}: Reports \name's accuracy in detecting various dental health problems including caries, calculus and food impaction. (2) \textbf{Sequence Alignment}: Presents \name's accuracy in identifying the correct tooth number brushed from audio signals; (3) \textbf{Benchmarking}: Considers the impact of various factors on system accuracy including brushing strength, duration, tooth location/type and ambient noise. 


\begin{figure*}
  \centering
  % \hspace{-0.1in}
  \begin{subfigure}[b]{0.25\linewidth}
    \includegraphics[width=\textwidth]{figures/foodstuck-userstudy.pdf}
    \vspace{-0.2in}
    \caption{\hspace{0mm}Food impaction (User Study)}
    \label{fig:food-user}
  \end{subfigure}
  \hspace{-0.1in}
  \begin{subfigure}[b]{0.25\linewidth}
    \includegraphics[width=\textwidth]{figures/foodstuck-model.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}Food Impaction (Model)}
    \label{fig:food-model}
  \end{subfigure}
  \hspace{-0.1in}
  \begin{subfigure}[b]{0.25\linewidth}
    \includegraphics[width=\textwidth]{figures/caries-userstudy.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}Caries (User Study)}
    \label{fig:caries-user}
  \end{subfigure}
  \hspace{-0.1in}
  \begin{subfigure}[b]{0.25\linewidth}
    \includegraphics[width=\textwidth]{figures/caries-model.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}Caries (Model)}
    \label{fig:caries-model}
  \end{subfigure}
  % \hspace{-0.1in}
  \newline
  \begin{subfigure}[b]{0.25\linewidth}
    \includegraphics[width=\textwidth]{figures/calculus.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}Calculus (User Study)}
    \label{fig:calculus-user}
  \end{subfigure}
  \begin{subfigure}[b]{0.28\linewidth}
    \includegraphics[width=\textwidth]{figures/loc-accuracy.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}Alignment accuracy}
    \label{fig:location-accuracy}
  \end{subfigure}
  \begin{subfigure}[b]{0.28\linewidth}
    \includegraphics[width=\textwidth]{figures/loc-error.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}Alignment Error}
    \label{fig:location-error}
  \end{subfigure}
  % \vspace{-0.1in}
  \caption{\name\ Results: (a) - (e) show the  ROC curves of the three health detection tasks. Three solid lines colored in blue, orange, and green show the detection performance using different number of cumulative measurements. The blue dashed lines show the performance of random choosing. (f) shows the accuracy of the sequence alignment to the correct tooth number. (g) shows the average alignment error of tooth number.  }
  % \vspace{-0.1in}
  \label{fig:overall-results}
\end{figure*}

\subsection{Health Detection}
We evaluate the health detection performance of \name\ using Receiver Operating Characteristic~(ROC) curve, which shows the detection sensitivity (True Positive Rate) versus False Positive Rate by varying the decision threshold. The Area Under Curve (AUC) value of the ROC curve represents \name's overall capability to distinguish unhealthy samples from healthy samples. We note that each measurement taken on the tooth of interest only lasts for 3-4~s, and 5-6~s for user study and dental model experiments respectively.

\sssec{Interdental Food Impaction:} We evaluate \name\ for the detection of interdental food impaction through the user study and on the dental model. We collected measurements on 26 teeth in total in the user study. As shown in Fig.~\ref{fig:food-user}, using a single measurement for around 3-4 seconds, \name\ achieves a 0.76 AUC value with a 95\% confidence interval of (0.702, 0.809). With 3 and 5 measurements, \name\ bootstraps the performance to 0.81~(0.783, 0.847), and 0.84~(0.744, 0.935) respectively.

We collected measurements on 20 dental model teeth with food impaction. As shown in Fig.~\ref{fig:food-model},  \name\ achieves a 0.76~(0.699, 0.821) AUC value using a single measurement. With three and five measurements, \name\ bootstraps the performance to 0.85~(0.821, 0.888), and 0.89~(0.792, 0.982) respectively. We note that the user study accuracy is slightly lower than the experiments on the model under multiple measurements mainly because some food is partially cleaned out during the data collection procedure.

\sssec{Caries Detection:} We evaluate \name\ for caries detection through the user study and on the dental model. We collected data on five teeth with caries from real patients during the user study and the results are shown in Fig.~\ref{fig:caries-user}. \name\ achieves 0.75~(0.637, 0.870), 0.86~(0.834,0.884), and 0.91~(0.893, 0.922) AUC values with 1, 3, and 5 accumulative measurements respectively. Similarly, we collected data on 10 teeth with caries on the dental model the results are shown in Fig.~\ref{fig:caries-model}, where it achieves a performance very close to the user study -- 0.77~(0.704, 0.835), 0.86~(0.848, 0.878), and 0.90~(0.894, 0.912) AUC values under 1, 3, and 5 measurements respectively.

\sssec{Caculus Detection:} We evaluate \name\ for caries detection only through the user study and on the dental model. We collected data on 30 teeth with calculus from real patients and the results are shown in Fig.~\ref{fig:calculus-user}. \name\ achieves 0.72~(0.663,0.768), 0.80~(0.768, 0.829), and 0.83~(0.738,0.920) AUC values with 1, 3, and 5 accumulative measurements respectively. Note that the dental calculus on the users who get dental cleaning frequently is generally very tiny, which induces smaller changes to the tooth resonances compared with caries or food impaction, so the detection performance is slightly lower.

\sssec{Accuracy vs. related work:}  OralCam~\cite{OralCam} is the only related work to \name\ that targets low-cost in-home dental health monitoring. OralCam reports 0.84, 0.79 AUC values for caries and calculus detection, which is close to the performance of \name\ using 3 measurements (0.86, 0.80 AUC), but lower than our results with 5 measurements (0.91, 0.83 AUC). We note OralCam evaluates on a visible disease dataset, but \name\ also has the unique advantage of detecting diseases at the most inner molars or even invisible corners where common cameras can hardly capture high-quality images.




\subsection{Sequence Alignment}
\label{subsec:sequence-alignment}
We evaluate the sequence alignment of \name\ through the user study on 90 teeth scanning sequences as shown in Fig.~\ref{fig:location-accuracy} and Fig.~\ref{fig:location-error}. We compare the results with the baseline warping algorithm which assumes the teeth scanning is performed at a uniform speed. We evaluate the alignment performance when the status of some of the teeth in the quadrant changes (e.g. food impaction) and without any changes compared with the status of the references. When the tooth status remains the same as the references, \name\ achieves an alignment accuracy of 82\% and an average error of tooth number 0.18, while the baseline algorithm has 68\% and 0.33 respectively. When the status of some of the teeth changes, \name\ achieves a 78\% localization accuracy and 0.21 average error of tooth number. The baseline algorithm achieves 62\% and 0.40 respectively. 

These results show the DTW algorithm in \name\ outperforms the naive algorithm on sequence alignment of teeth scanning. Also, the alignment performance only degrades slightly when tooth status changes since the selected features for the sequence alignment algorithm are designed to be resilient to health condition changes.

\begin{figure*}
  \centering
  % \hspace{-0.1in}
  \begin{subfigure}[b]{0.25\linewidth}
    \includegraphics[width=\textwidth]{figures/strength.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}Brushing strength}
    \label{fig:strenght}
  \end{subfigure}
  \hspace{-0.1in}
  \begin{subfigure}[b]{0.25\linewidth}
    \includegraphics[width=\textwidth]{figures/testlength_new.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}Duration of brushing}
    \label{fig:testlength}
  \end{subfigure}
  \hspace{-0.1in}
  \begin{subfigure}[b]{0.25\linewidth}
    \includegraphics[width=\textwidth]{figures/caries-lower-vs-upper.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}Lower vs. Upper Teeth}
    \label{fig:lowerVsUpper}
  \end{subfigure}
  \hspace{-0.1in}
  \begin{subfigure}[t]{0.26\linewidth}
    \vspace*{-1.2in}
    \includegraphics[width=\textwidth]{figures/loc-parts.pdf}
    \vspace{-0.1in}
    \caption{\hspace{0mm}Types of Teeth}
    \label{fig:loc-parts}
  \end{subfigure}
  % \vspace{-0.1in}
  \caption{Evaluation results of different factors. (a) compares the detection accuracy under different brushing strengths. (b) compares the detection accuracy of different duration of brushing on a single tooth. (c) shows the ROC curve of detection performance on upper teeth v.s. lower teeth. (d) shows the alignment error on different types of teeth (Inc\&Cus: Incisors and Cuspids). }
  % \vspace{-0.1in}
  \label{fig:overall-results}
\end{figure*}


\subsection{Benchmarking}
\label{subsec:benchmark}
\sssec{Brushing Strength:} In this experiment, we study how the brushing strength affects the detection accuracy of food impaction detection on the dental model in Fig.~\ref{fig:strenght}. This study shows slight changes in accuracy when brushing strength varies, showing that \name\ is robust to different brushing behavior. Interestingly, the detection accuracy increases as the brushing strength increases when \name\ has enough measurements (5 times). As the strength increases, the brush bristles have closer and tighter contact with the brushed tooth, which in turn produces a response resonances with a higher signal-to-noise ratio.


\sssec{Brushing Duration:} We evaluate in this experiment how the duration of each brushing measurement on a single tooth affects the detection accuracy of food impaction in the user study. \name\ seeks to average the tooth signatures from the same tooth across multiple time windows to improve the signal-to-noise ratio (Sec.~\ref{sec:alignment}). As Fig.~\ref{fig:testlength} shows the detection accuracy increases as the brushing duration increases for each tooth as expected, achieving relatively good performance when the duration reaches 3-4 seconds, which is also the chosen duration in our user study.


\sssec{Upper vs. Lower Teeth:} We compare the detection accuracy of caries on the dental model for the upper teeth versus the lower teeth. Fig.~\ref{fig:lowerVsUpper} shows \name\ achieves a better detection performance on lower teeth (AUC = 0.94) compared with upper teeth (AUC = 0.86). Brushing upper teeth is usually more challenging as the applied force is in the opposite direction of gravity. As a result, the brush head generally has better contact with the lower teeth leading to better detection performance. 
% Fig.~\ref{fig:lowerVsUpper} shows significant improvement for the detection accuracy when moving from brushing the upper teeth (AUC = 0.86 AUC) to brushing the bottom teeth (AUC = 0.94). Brushing the upper teeth is usually challenging compared to the lower teeth as it's easier to see what are brushing for the lower teeth. Moreover, food debris fall off from the upper to the lower part of the mouth, resulting in clear changes for \name\ to detect.


\sssec{Types of Teeth:} In this experiment, we show how the different types of teeth, like Incisors, Cuspids, Premolars, and Molars, affect the alignment error. Fig.~\ref{fig:loc-parts} shows the mean error of detecting the tooth number that the user is currently brushing, and how it varies over different types of teeth. 
Since the premolars are generally smaller and have irregular non-flat shapes compared with other teeth, it introduces slightly higher alignment errors. 
% As the molars are hard to reach and brush properly, it is also challenging to align them. This also similar to the incisors and cuspids, as it's challenging to brush each of them separately given their size is usually smaller than the brush head itself.



\begin{figure*}[h]
  \centering
  % \hspace{-0.1in}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\textwidth]{figures/emd-1time.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}1-Time Measurement}
    \label{fig:emd-1time}
  \end{subfigure}
  % \hspace{-0.15in}
  \begin{subfigure}[b]{0.3\linewidth}
    \includegraphics[width=\textwidth]{figures/emd-5time.pdf}
    \vspace{-0.2in}
    \caption{\hspace{1mm}5-Times Measurements}
    \label{fig:emd-5time}
  \end{subfigure}
  % \vspace{-0.1in}
  \caption{Noise Suppression Evaluation: We compare the calculus detection performance in the user study with and without the denoised algorithms in Sec.~\ref{subsec:noise-suppression}}
 % \vspace{-0.2in}
  \label{fig:emd-eval}
\end{figure*}


\sssec{Noise Suppression:} We illustrate in this experiment how the Noise Suppression module (Sec.~\ref{subsec:noise-suppression}) affects the system performance. We present the accuracy of the food impaction detection in our user study, as it is conducted in a comparatively noisy environment with surrounding speech.  As shown in Fig.~\ref{fig:emd-eval}, our Noise Suppression module can significantly improve the detection accuracy. Further, \name\ improves the detection accuracy of calculus, in terms of AUC values, from 0.69 to 0.76, and from 0.75 to 0.84, for 1-time and 5-times accumulative measurements, respectively.

\subsection{Expert Evalution}\label{sec:expert}

To evaluate \name\ from the expert's point of view, we interviewed 2 board-certified dentists (D1 \& D2). D1 has 30 years of practice with expertise in restorative dentistry, and D2 has 8 years of practice with expertise in oral radiology. We investigated the following questions:
\begin{enumerate}
    \item Is our current data collection procedure valid? What would be your recommendations to improve the data collection procedure for our system?
    \item What is your opinion of the current performance of our system?
    \item What are the potential benefits of integrating this technology into the current dental healthcare system? What are the main limitations and barriers?
\end{enumerate}

\sssec{Data collection procedure:} Both dentists agreed that our data collection procedure is sufficient and valid. For the recommendations, D2 points out the importance of collecting data from caries evolving at different stages, which can be left as future work. D2 mentioned: "\textit{If they are really small caries, we don't care. If they're really big carries, we can actually see it and be fine. So this becomes very useful when we can detect those in-between carries. But that will be a much harder data collection.
}" Besides, D1 suggested exploring the prototype of toothbrush heads that are designed for actual detection rather than existing ones designed for hygiene.

\sssec{System Performance:} Both dentists stated that the overall detection accuracy of our system is promising, especially considering our current system is just using a regular toothbrush without specialized hardware. Meanwhile, both dentists agreed that, from a clinical point of view, it is necessary to further optimize the system and improve its accuracy. D2 mentioned: "\textit{I think the results are promising... When using cumulative 5 times measurements, the accuracy is consistently high... But we will have to tweak everything. The calculus one with one-time measurement seems to work at 0.72, which is not decent.}"

\sssec{Benefits to current dental healthcare system and potential barriers:} Both dentists considered that the potential of at-home early caries detection of our system is beneficial to the dental healthcare system, since it can catch caries earlier, prevent more severe diseases from happening and reduce the overall costs of the system. D1 also mentioned detecting unseen food impaction will have a direct impact on the patient's overall periodontal health. D2 emphasized the importance of at-home dental calculus detection: "\textit{We recommend the patient do come for a checkup every 6 months, but in practicality that is not possible for a lot of people. So having that calculus detection system will also again help the patient understand that there's some issue going on, and they need to go to the dentist and get it fixed before it becomes a much bigger issue, such as periodontal bone loss.}"

For the potential barriers, D2 is concerned about the accessibility of our system to low-income families. Families without access to regular dental visits may also lack powerful enough smartphones to receive and process the data. D1 is concerned about the interpretation of data by the patients and suggests the actual system can present the result by incorporating the dentist's interpretation. 

==> Implementation.tex <==
\section{Implementation and Evaluation}



\sssec{Implementation:} We implement \name\ on a Philips Sonicare ProtectiveClean 6100 electric toothbrush~\cite{sonicare6100} and a Voice Technologies VT500X waterproof microphone~\cite{vt500x}. For toothbrush heads, we choose Brushmo Compact Replacement Heads~\cite{brushmo} as it has a smaller size compared with the standard one. As shown in Fig.~\ref{fig:hardware}, the microphone is fixed 1.25~cm close to the toothbrush head using a tiny glass stick, which is integrated onto the toothbrush body. The microphone is sampling at 44.1~kHz for audio recording and connected to a laptop through a 3.5~mm audio jack. A video camera is put in front of user's mouth to capture the real-time ground truth locations of the toothbrush. Note that the camera is only needed as ground truth for the evaluation of sequence alignment -- \name\ does not require or rely on camera data. We use an online video labeling tool~\cite{Labelbox} to label the tooth being brushed in each video frame.

For signal processing, we choose a 50 milliseconds time window and 75\% overlap to perform STFT. For signals from users and dental models, we empirically choose the frequency range of 2-16~kHz, and 2-18~kHz respectively to obtain the cepstrum (illustrated in Sec.~\ref{subsec:extract-alg}).

\sssec{Evaluation through user study:} We conducted an IRB-approved user study on 19 participants (12 males and 7 females). We evaluated the health detection for caries and calculus in a dental clinical center, where we perform measurements on real patients under the guidance of professional dentists. For the evaluation of caries detection, we took measurements on specific teeth with caries (labeled by dentists) before and after the dental fillings (example shown in Fig.~\ref{fig:caries-photo}). For the evaluation of calculus detection, we perform measurements on teeth originally with calculus before and after the dental cleaning (example in Fig.~\ref{fig:calculus-photo}). For every tooth of interest from every patient, we collected 10 measurements each before and after the treatments (20 measurements in total). We assume the teeth after the treatments are healthy, use a subset of samples (5 measurements) after the treatments as references, and test on the rest of the samples (15 measurements). We use random combinations of 3 or 5 measurements among the 15 measurements to evaluate the multi-measurement bootstrapping as presented in Sec.~\ref{sec:detection}.

We also evaluated detection for interdental food impaction in a home setting. We collected measurements on the original normal teeth, teeth with food impaction after eating, and the teeth after flossing to clear out impacted food. We collected 10 measurements in each stage (30 measurements in total) for every tooth of interest from every participant. We use 5 measurements from the original normal teeth as references and test on the others.

\sssec{Evaluation on dental models:} We further increase the scale of the evaluation by using professional dental models designed for dental training. We perform this evaluation to allow for more controlled damage to be performed on the teeth, unlike a relatively more unstructured user study context. We use an electric drill to produce small holes on the surface of the model's teeth to emulate caries, and insert meat samples in between two teeth to emulate food impaction (shown in Fig.~\ref{fig:model-photo}). We collect measurements on the model teeth before and after the changes for our evaluation. The number of measurements on each tooth of interest is the same as in the user study.



